The density distribution and physical origins of intermittency in supersonic, highly magnetised turbulence with diverse modes of driving

The probability density function (PDF) of the logarithmic density contrast, $s=\ln (\rho/\rho_0)$, with gas density $\rho$ and mean density $\rho_0$, for hydrodynamical supersonic turbulence is well-known to have significant non-Gaussian (intermittent) features that monotonically increase with the turbulent Mach number, $\mathcal{M}$. By studying the mass- and volume-weighted $s$-PDF for an ensemble of 36 sub-to-trans-Alf\'venic mean-field, supersonic, isothermal turbulence simulations with different modes of driving, relevant to molecular gas in the cool interstellar medium, we show that a more intricate picture emerges for the non-Gaussian nature of $s$. Using four independent measures of the non-Gaussian components, we find hydrodynamical-like structure in the highly magnetised plasma for $\mathcal{M} \lesssim 4$. However, for $\mathcal{M} \gtrsim 4$, the non-Gaussian signatures disappear, leaving approximately Gaussian $s$-statistics -- exactly the opposite of hydrodynamical turbulence in the high-$\mathcal{M}$ limit. We also find that the non-Gaussian components of the PDF increase monotonically with more compressive driving modes. To understand the $\mathcal{M} \lesssim 4$ non-Gaussian features we use one-dimensional (1D) pencil beams to explore the dynamics along and across the large-scale magnetic field, $\mathbf{B}_0$. We discuss kinetic, density and magnetic field fluctuations from the pencil beams, and identify physical sources of non-Gaussian components to the PDF as single, strong shocks coupled to fast magnetosonic compressions that form along $\mathbf{B}_0$. We discuss the Gaussianisation of the $\mathcal{M} \gtrsim 4$ $s$-fields through the lens of two phenomenologies: the self-similarity of the $s$-field and homogenisation of the dynamical timescales between the over- and under-dense regions in the compressible gas.

==> space_time.tex <==
\begin{figure*}
    \centering
    \includegraphics[width=\linewidth]{Figures/spaceTime_Ma01_zoomin.pdf}
    \caption{\textbf{Top:} The same as Figure \ref{fig:spacetimeIso} but for the \texttt{M2MA01} (left) and \texttt{M20MA01} (right) simulations, with time orientated up the page, a space across the page. We show $\rhoperp$ and $\rhopar$ decompositions, labelled in the top-right corner for each of the panels. In addition to characteristics shown in Figure \ref{fig:spacetimeIso}, we show $v = v_{\rm A 0}$, indicated with the dashed white line, in each of the panels, indicating that waves travelling at $v_A$ are close to horizontal in these space-times. We see structurally different space-time diagrams between the two different density decompositions for both simulations, suggesting that we are capturing different types of density fluctuations with our decomposition method. \textbf{Bottom:} A zoom-in of the first $5\,T$ from the left plot in top panel. These compressions in the density follow the fast magnetosonic speed characteristics, shown with the white-dashed lines. The fluctuations have extremely short lifetimes, much less than a single turbulence turnover time.}
    \label{fig:spacetimesAniso}
\end{figure*}

\begin{figure*}
    \centering
    \includegraphics[width=\linewidth]{Figures/spaceTime_M4.png}
    \caption{Space-time diagrams for the density decomposition of the isotropic \texttt{M4} simulation, shown in Table \ref{tb:simtab}. Space is shown in units of $L$ in along the $y$-axis, and time in units of $T$, along the $x$-axis, evolving from left-to-right. White characteristics for $v = 4c_s$ (the rms $\M$), tracing shock structures, and $v = c_s$, tracing more diffuse structures. The perpendicular component of the field (top) and parallel component of the field (bottom) appear statistically similar, indicating that the space-time diagram is invariant to different 1D projections of the 3D field for the isotropic, hydrodynamical case.}
    \label{fig:spacetimeIso}
\end{figure*}


\section{Unravelling the anisotropic density fluctuations}\label{sec:densDecomp}

    In this section we discuss how one can decompose a scalar field into fluctuating components along and perpendicular to the mean magnetic field for our simulations. First we create a set of one-dimensional (1D) fluctuations along each coordinate axis, turning our 3D field into a set of three 1D fields,
    \begin{align}
        \rho_x(x) = & \frac{1}{N_y N_z}\int_{-L_y/2}^{L_y/2}\int_{-L_z/2}^{L_z/2} \d{y\d{z}} \, \rho, \\
        \rho_y(y) = & \frac{1}{N_x N_z}\int_{-L_x/2}^{L_x/2}\int_{-L_z/2}^{L_z/2} \d{x\d{z}} \, \rho, \\
        \rho_z(z) = & \frac{1}{N_x N_y}\int_{-L_y/2}^{L_y/2}\int_{-L_x/2}^{L_x/2} \d{x\d{y}} \, \rho,
    \end{align}
    where $N_x = N_y = N_z = 512$ are the amount of grid cells in a single dimension for our simulations. The mean magnetic field in our simulations is along the $z$-axis, which we can use to define the parallel component of the density field,
    \begin{align} \label{eq:rhoPar}
        \rhopar = \rho_z(z,t),
    \end{align}
    and the cylindrical symmetry of the system gives a canonical definition for the perpendicular density component,
    \begin{align} \label{eq:rhoPerp}
        \rhoperp = \rho_x(x,t) = \rho_y(y,t),
    \end{align}
    which we mean in the statistical sense. Using these definitions we can construct a set of space-time diagrams that allow us to probe spatial scales along and across $B_0$. We discuss these turbulent space-times, their power spectra, PDFs, and variances in the next few sections.
    
    \subsection{Turbulent Space-time diagrams}

    We plot the 1D space-time diagrams of the fluctuations in Figures \ref{fig:spacetimeIso} and \ref{fig:spacetimesAniso}. Figure \ref{fig:spacetimeIso} shows the space-time diagram for the \texttt{M4} simulation, which is hydrodynamical and isotropic, where space is along the $y$-axis and time along the $x$-axis. Like any space-time diagram, we have a set of characteristics that tell us velocity information about how the 1D density structures propagate in time. Using Equation~(\ref{eq:T(M)}) we plot the characteristics for when $v = \text{rms}\,\M$, and $v = c_s$, and show them in white in Figure \ref{fig:spacetimeIso}.
     
    We see that our decomposition produces a similar space-time diagram for both the $\rhoperp$ (Equation~\ref{eq:rhoPerp}) and $\rhopar$ (Equation~\ref{eq:rhoPar}) fields for the \texttt{M4} simulation. This is to be expected for an isotropic density field, where any space-time diagram should be statistically similar to any other. The 3D-1D decomposition of the field preserves some structure of the 3D simulations. For example, we see sharp shock structures travelling through the field, roughly following the $v = 4c_s$ characteristic. We also observe rarefaction waves, or voids, reminiscent of the voids that we observe in compressively-driven 3D turbulence \citep{Federrath2008} forming in 1D, and propagating at roughly the $v = c_s$ through the simulation. The same is true for the more diffuse structures, which mostly fall within the $v = c_s$ cone. Hence, the diffuse, and rarefactions travel close to the sound-speed, and the high-density, shocked structures travel close to the rms $\M$. We now show how when we introduce a magnetic field we get more than a single (statistically similar) space-time diagram for the density field. 
     
    In Figure \ref{fig:spacetimesAniso} we show four space-time diagrams for the \texttt{M2MA0.1} (left two panels) and \texttt{M20MA0.1} (right two panels) simulations. In the first panel for each Mach number we show the $\rhoperp$ data, and the second is the $\rhopar$ data. For both of the simulations we see qualitatively different structures in the $\rhoperp$ and $\rhopar$ decomposition. 
    
    \subsubsection{Fast magnetosonic waves in the \texttt{M2MA0.1} simulation}\label{sec:M2MA01sim}
    
    The difference between the two different decompositions may be most obvious in the \texttt{M2MA0.1} simulation. In the $\rhoperp$ space-time diagram we see only very small amplitude fluctuations compared to $\rhopar$, and between 0-5$\,T$ we see waves that are almost horizontal in the diagram. We plot the Alfv\'en velocity for comparison, shown with the white-dashed line which reveals that these waves are travelling $\mathcal{O}(v_{\text{A}})$. We zoom into this region further in the bottom panel of Figure \ref{fig:spacetimesAniso}, and show the fast magnetosonic speed (Equation~\ref{eq:fastVelocity}) with the white characteristics. Since these waves are travelling perpendicular to the magnetic field and have a velocity typical of fast magnetosonic waves we identify these waves as fast magnetosonic waves in the space-time diagrams. These density fluctuations have extremely small lifetimes, only persisting for a few tenths of $T$.
    
    As shown in Figure~\ref{fig:spacetimesAniso} these waves dominate the space-time diagram until fluctuations associated with the turbulence leak into $\rhoperp$. This is simply a measure of the success of our decomposition, which is not perfect, but clearly does a reasonable job by capturing the projected, fast magnetosonic waves. 
    
    In the $\rhopar$ decomposition we see a network of interacting shocks, travelling along the $v = 2c_s$ characteristics (the rms $\M$ of the simulation). The space-time diagram shares similar properties to the hydrodynamical space-time diagrams in Figure~\ref{fig:spacetimeIso}, suggesting that we have captured the hydrodynamical component of the magnetised density field.
    
    \subsubsection{Shocks in the \texttt{M20MA0.1} simulation}
    
    \begin{figure}
        \centering
        \includegraphics[width=\linewidth]{Figures/shock_edges_M20.pdf}
        \caption{\citet{Canny1986} edge detection algorithm applied to the $\rho_{\parallel}$ space-time diagram for the \texttt{M2MA0.1} simulation. The edge features reveal a wealth of strong shocked structures travelling through the turbulent space-time at $\M \approx 20$. The space-time diagrams discussed in this study have some resemblance to directed percolation diagrams in a fully turbulent Couette experiment, but instead of describing turbulent and laminar regions, as done in \citet{Lemolt2016}, here we map out shocked and rarefaction regions -- fundamental building blocks of supersonic turbulence.}
        \label{fig:shockEdges} 
    \end{figure}
    
    The $\rhoperp$ component for the \texttt{M20MA0.1} simulation is more contaminated with shocks than the  \texttt{M2MA0.1} simulation. This is because the turbulence is so strong that on large scales (small $k$ modes) it remains isotropic \citep[see discussion in \S4.3.2]{Beattie2020}. This prevents the space-time revealing the density fluctuations caused by magnetosonic waves when the turbulence is significantly supersonic. A qualitative difference between the $\rhoperp$ and $\rhopar$ space-time diagrams is, however, still noticeable. For example, the interacting density structures in the $\rhoperp$ direction are much more volume-filling than in the $\rhopar$ data. The amount of compression, and hence the development of shocks and voids, reduce the volume-filling factor of the flow \citep{Federrath2009,Beattie2019a}. This suggests that even though we do not completely decouple the density field in the high-$\M$ simulations, we still decompose some dynamically different behaviours in the density field. 
    
    The shocks are more clearly resolved in the \texttt{M20MA0.1} simulation because of the large density contrasts that scale with $\sim \M^2$. Some of the dense shock-like structures persist for $\gtrsim 1\,T$, which is much longer than the time-scales measured for the lifetime of shocked regions in supersonic, hydrodynamical turbulence \citep{Robertson2018}. We use a \citet{Canny1986} edge detection algorithm to more clearly extract the shock structures in Figure~\ref{fig:shockEdges}. For a real molecular cloud, $T \sim \mathcal{O}(\text{Myr)}$, with cloud collapse happening roughly at the same dynamical time scale \citep{Federrath2012,Federrath2015a}. To be more precise, the free-fall time of an MC can be written in terms of the turbulent turnover time,
    \begin{align}
        \tff \propto (G\rho_0)^{-1/2} \propto \alpha_{\text{vir}}^{-1/2}\M^{-1} \propto c_s L^{-1}\alpha_{\text{vir}}^{-1/2} T,  
    \end{align} 
    where $\alpha_{\text{vir}} \sim 1$ for virialized clouds \citep{Heyer2015a} and the proportionality factor is $\ll 1$ \citep{Mocz2018}. This means that density structures that persist for longer than a turnover time (let alone a couple) have the appropriate dynamical timescale for collapse, and eventually star formation to occur. \citep{Robertson2018} provides a much more detailed analysis of the timescales involved with dense regions in hydrodynamical turbulence and finds that shocks and dense regions only persist for a small fraction of the global dynamical time (sound-crossing time, which is two turnover times in our units). Our results suggest that magnetic pressure significantly increase the lifetime of the dense regions, qualitatively found previously in \citet{Hennebelle2012}. Being able to easily identify such timescales is a very nice property of the space-time decomposition, but of course one has to be careful with concluding anything too strongly since projecting the 3D fields to 1D can significantly influence the field, which we discuss in \S\ref{sec:proj}. Next we discuss a more conventional measure for studying the fluctuations in these anisotropic space-time diagrams, the 1D power spectrum.
    
    \begin{figure}
        \centering
        \includegraphics[width=\linewidth]{Figures/powerSpec.pdf}
        \caption{\textbf{Top:} The power spectra of the parallel (black) and perpendicular (red) isotropic \texttt{M4} space-time. \textbf{Bottom:} The same as the above panel except for the power spectra of the $\Mao = 0.1$  space-time diagrams. Each of the power spectra are offset by 7.5 dex to reveal how the density fluctuations change as a function of $\M$.}
        \label{fig:powerSpec}
    \end{figure}
    
    % \begin{figure*}
    %     \centering
    %     \includegraphics[width=\linewidth]{Figures/3DDis.pdf}
    %     \caption{3D $s$-PDFs for the $\Mao = 0.1$ simulations from Table \ref{tb:simtab}.  \pmocz{In upper plot, what would pure-hydro prediction look like? (ideally an upper bound) pure fast-wave prediction? (ideally a lower bound) } }
    %     \label{fig:3Ddensity}
    % \end{figure*}
     
    \subsection{Space-time power spectra}

    % \subsubsection{Contextualising the power spectra}
    
    % Before describing in detail the 1D power spectra of the space-time diagrams discussed previously we should clarify what taking a power spectrum of this dataset really means. First let us consider the 3D density $\rho/\rho_0$, being averaged onto a 2D plane, i.e. the mean line-of-sight (LOS) projection, $\Sigma / \Sigma_0$. The slice - projection theorem, commonly used in medical imaging \citep[e.g.][]{Levoy1992,Bom2010} but also in various astrophysical studies \citep{Brunt2010a,Brunt2010b}, states that the relation between the density Fourier transforms of the density field is\footnote{Note that this is for the mean LOS, and not simply the projection, which is usually referred to as the column density. If one is to consider the column density, and not the mean LOS then the relation $\mathscr{F}_{\rho/\rho_0}(k_x,k_y,k_z=0) = \mathscr{F}_{\Sigma/\Sigma_0}(k_x,k_y)$ holds.}, 
    % \begin{align}
    %     \frac{1}{L}\mathscr{F}_{\rho/\rho_0}(k_x,k_y,k_z=0) = \mathscr{F}_{\Sigma/\Sigma_0}(k_x,k_y), 
    % \end{align}
    % and then the 1D projection onto the $x$-axis is further,
    % \begin{align} 
    %     \frac{1}{L}\mathscr{F}_{\Sigma/\Sigma_0}(k_x,k_y=0) = \mathscr{F}_{\rho_x / \Exp{\rho_x}}(k_x), 
    % \end{align}
    % hence the relation between the 3D and 1D field is,
    % \begin{align}
    %     \frac{1}{L^2}\mathscr{F}_{\rho/\rho_0}(k_x,k_y=0,k_z=0) = \mathscr{F}_{\rho_x / \Exp{\rho_x}}(k_x). 
    % \end{align}
    % Squaring both sides of this equation gives us the relation between the power spectra of the 3D field and the 1D projection,
    % \begin{align}
    %     \frac{1}{L^4}\mathscr{P}_{\rho/\rho_0}(k_x,k_y=0,k_z=0) = \mathscr{P}_{\rho_x / \Exp{\rho_x}}(k_x),
    % \end{align} 
    % where $\mathscr{P}_{f} \equiv \mathscr{F}_{f}^2 = \mathscr{F}_{f}\mathscr{F}^*_{f}$, for arbitrary function $f$, and $\mathscr{F}^*_{f}$ is the complex conjugate of the Fourier transform. This means that the power spectra of the 1D space-time diagrams is a scaled slice through the 3D power spectrum. This means that the power spectra of the space-time diagrams are representative of slices through the 3D power spectra along and perpendicular to the magnetic field, defining the principle axis of the elliptical structures studied in \citet{Beattie2020}. Now that we understand the relation between the 3D and 1D power spectra we discuss the construction and results.

    \subsubsection{Construction}
    We define the 1D space-time power spectra as
    \begin{align}\label{eq:PS}
        \mathscr{P}_{\rho/\rho_0}(k) =  \frac{1}{N^2} \left(\displaystyle\sum^{N-1}_{x = 0} \frac{\rho}{\rho_0}(x) \exp\left\{ -i\frac{xk}{N}  \right\}\right)^2, 
    \end{align}
    where we use $\rho/\rho_0$ to indicate either the $\rhopar/\Exp{\rhopar}$ or $\rhoperp/\Exp{\rhopar}$ variable, $N$ is the 1D grid size and $i \equiv \sqrt{-1}$. As is the case for the study of many turbulent systems, we identify a scaling range in the power spectrum that is linearised under the log-log transform, i.e. the region in $k$-space where the power spectrum takes the form,
    \begin{align}
        \mathscr{P}_{\rho/\rho_0}(k) \sim k^{\alpha}.
    \end{align}
    For our simulations this region lies roughly between $10 \leq k \leq 30$, consistent with other studies of the density power spectra \citep{Federrath2013}. We construct the power spectra for the space-time diagrams of each simulation, and plot the median, 10th and 90th quantile from $5 - 10\,T$ in Figure \ref{fig:powerSpec}. We also use least-squares to fit linear models of the form $\log_{10}\mathscr{P} = \log_{10} \beta + \alpha \log_{10} k$, where $\beta$ and $\alpha$ are the fit parameters, to the each of the space-time realisations between $5 - 10\,T$, revealing the power-law index, $\alpha$, for each of the experiments, and report the median, 10th and 90th quantile in Figure \ref{fig:powerSpecExp}.
    
    \begin{figure}
        \centering
        \includegraphics[width=\linewidth]{Figures/powerSpecExponents.pdf}
        \caption{The power-law exponents for the $\mathscr{P}_{\rho/\rho_0}(k) \sim k^{\alpha}$ fits from the power spectra in Figure \ref{fig:powerSpec}. We fit on wavenumbers $10 \leq k \leq 30$. Values of $\alpha$ towards the top of the plot indicate a shallow power spectra with significant power in the high-$k$ modes. For $\alpha$ values towards the bottom of the plot the spectra is more large-scale, with most of the power in low-$k$ modes. }
        \label{fig:powerSpecExp}
    \end{figure}
    
    \subsubsection{Results}
    
    In the top panel of Figure \ref{fig:powerSpec} we find both the $\rhopar$ and $\rhoperp$ power spectra aligned perfectly with one another. This is to be expected in the isotropic case, where fluctuations are not dynamically distinct from one another, in any direction. In the bottom panel Figure \ref{fig:powerSpec} we show the anisotropic simulations, increasing in $\M$ from bottom-to-top. As $\M$ increases we find that only the $\rhopar$ power spectrum shallows, and the $\rhoperp$ spectrum stays roughly constant. This can be seen in the scaling exponents of the spectra, shown in Figure~\ref{fig:powerSpecExp}. The transition from large-scale to small-scale field is a well-known property of hydrodynamical turbulence \citep{Kim2005}. This is caused by the introduction of small-scale fluctuations in the field as the $\M$ increases, shifting more power to high-$k$ modes and shallowing the spectra. Because this phenomena is only found in the $\rhoperp$ spectra this is more, strong evidence for the model we propose in \S\ref{sec:twoShockModel}, where the hydrodynamic component is completely encapsulated in $\rhoperp$.
    
    
    \begin{figure*}
        \centering
        \includegraphics[width=\linewidth]{Figures/anisoPDF.pdf}
        \caption{The normalised (mean = 0, variance = 1) volume-weighted PDFs for the perpendicular (black; $\rhoperp$) and parallel (red; $\rhopar$) density fluctuations, with respect to the mean magnetic field. We show a standardised Normal distribution, $\mathcal{N}(0,1)$, in blue for comparison between the structure of the PDFs, and fit a $\mathcal{CN}$ (Equation~\ref{eq:CNdis}) to the $\rhoperp$ PDF, shown in orange. The $\rhopar$ PDFs approximately follow Normal distributions, whereas the $\rhoperp$ have two notable components: the first component is the $\mathcal{CN}$ distribution, from the magnetised density fluctuations, and the second component is the low-density tails, which comes from eddies that form perpendicular to the magnetic field.}
        \label{fig:pdfs}
    \end{figure*}     
    
    \begin{figure*}
        \centering
        \includegraphics[width=\linewidth]{Figures/projections_comp_landscape.pdf}
        \caption{An example of the fluctuations in the plane perpendicular to the magnetic field for the \texttt{M2MA01} (left) and \texttt{M20MA01} (right) simulations, both shown at the same time-realisation, $t = 6\,T$. \textbf{Left:} The lowest density values are from eddies that develop, creating low-pressure regions in the field and contributing to the low-density tail in the top-left PDF in Figure \ref{fig:pdfs}. A signature of the eddy can also be seen in the low-density streak through the left-most space-time diagram in Figure \ref{fig:spacetimesAniso}. The size of the eddy corresponds approximately to the sonic scale, $\sigma_v(\ell=\ell_s) = c_s$, indicated with the circle in the lower-left. \textbf{Right:} Strong-shocks shred eddies that form in the density field, and dominate the structure in the high-$\M$ simulations, creating an approximately log-Normal $\rhoperp$ distribution for the density fluctuations. }
        \label{fig:eddy}
    \end{figure*}
    
\subsection{Space-time density PDFs}\label{sec:stPDFs}
    We construct density PDFs for each of the space-time diagrams, averaging over the statistically stationary data. We show the $s\equiv\ln(\rho/\rho_0)$ PDFs in normalised (mean $=0$, variance $= 1$) form, organised by $\M$ in Figure~\ref{fig:pdfs} and discuss the low-$\M$ and high-$\M$ simulations separately in the following sections. 
    
    \subsubsection{$\M = 2 - 4$}
    In the top two panels of Figure~\ref{fig:pdfs} we show the low-$\M$ simulations from our ensemble. The $\rhopar$ distributions (shown in black) roughly follow a log-Normal distribution, which we show overlaid in blue. This is of course typical of hydrodynamical turbulence, as discussed in \S\ref{sec:logNormal}, and what we should expect for many, largely-uncorrelated density fluctuations. The $\rhoperp$ PDFs, however, shows a distribution with two components, with something that resembles a Gaussian with intermittent wings centred at the mean, and then an extended low-density tail. 
    
    An extended negative tail has been observed before in magnetic field distributions for low-$\M$ simulations in \citet{Beattie2020c}. These are caused by low-magnetic pressure, low-density vortexes (or eddies) in the flow that cause magnetic field fluctuations that oppose $B_0$. Here we add that these eddies contribute to the structure of the density PDF perpendicular to $B_0$. A visualisation of the eddy can be seen projected onto the perpendicular plane to $B_0$ in Figure~\ref{fig:eddy}. The time-evolution of the eddy can be seen in the in the left space-time diagram in Figure~\ref{fig:spacetimesAniso} as a low-density streak moving through the magnetised fluctuations and sustaining itself for over $5\,T$ in the turbulence.
    
    The eddy is roughly $L/4$ in diameter or $\ell_{\rm D}/2$. This marks the shock width scale $\ell_s = L/\M^2 = L/4$, which also roughly corresponds to sonic scale of the turbulence, i.e. the scale where $\sigma_v(\ell = \ell_s) = c_s$, where $\sigma_v(\ell)$ is the velocity dispersion on the scale $\ell$. This is the scale where the pressure gradient, $c_s^2\nabla\rho$, becomes dynamically important. It is possible that the local, low pressure system sucks in more magnetic field lines, increasing the magnetic field and providing a magnetic shield against the large-scale shocks. Such extended life times have been found previously in magnetised filaments \citep{Hennebelle2013}.
    
    % Since these highly-magnetised eddies are so long-lived, well-beyond a free-fall time, they may be able to be observed in MCs with the mean-field component of the cloud parallel with the line-of-sight (LOS), but however, since they seem to be below the sonic scale, which $~0.1\text{pc}$ for a typical MC, there small rotational velocities may not be detectable.
    
    For the component of the PDF that is centred around the mean we fit $\mathcal{CN}$ distribution, shown in yellow, as shown in Equation~(\ref{eq:CNdis}). This captures the intermittent density fluctuations that we associate with fast magnetosonic waves. The intermittency in the fluctuations comes about directly from (1) the intermittent magnetic field fluctuations (see Figure 8 of \citealt{Beattie2020c} and \S3 in \citealt{Seta2020}) and (2) the strong correlation with the magnetic field ($B \propto \rho$ for fast magnetosonic waves, which comes directly from the shock-jump conditions). The $\mathcal{CN}$ helps to guide the eye and show how the $\rhoperp$ and $\rhopar$ are distinct from one another. However, as $\M$ increases the log-Normal and $\mathcal{CN}$ distributions take on parameter values that converge to same morphology.
    
    \subsubsection{$\M = 10 - 20$}
    With increasing $\M$ the $\rhoperp$ fluctuations become log-Normal as the eddies found in the lower-$\M$ turbulence are sheared and destroyed by large-scale shocks. We show this for the same This causes $\rhoperp$ and $\rhopar$ distributions to converge on a log-Normal form, as shown in the lower panel of Figure~\ref{fig:pdfs} where the $\mathcal{CN}$ becomes $\sim \mathcal{N}(0,1)$. In normalised form, these distributions are identical and so now we turn to the magnitude of the variance. 
    
    \begin{figure}
        \centering
        \includegraphics[width=\linewidth]{Figures/var_frac.pdf}
        \caption{\textbf{Top:} The density variance of the $\rhopar/\rho_0$ (black) and $\rhoperp/\rho_0$ (red) for the 1D space-time diagrams for each of the sub-Alfv\'enic simulations from Table~\ref{tb:simtab} as a function of $\M$. \textbf{Bottom:} The ratio between the total (3D volume) variance and the variance from the 1D space-time diagrams, showing how the variance is influenced by projecting the 3D data onto a one-dimensional line. For the $\rhoperp$ field the projection effect is almost constant for all $\M$, however for the $\rhopar$ field the projection effect monotonically decreases the variance.}
        \label{fig:1Dvariances}
    \end{figure}

    \subsubsection{Variances and projection effects}\label{sec:proj}
    The value of the variance is not captured when the PDFs are shown in normalised form. However, it is this value that tells us the total power in the fluctuations, which we associate with different dynamical behaviour. We show the magnitude of the variance for each of the distributions in Figure~\ref{fig:1Dvariances}. The $\sigma^2_{\rhopar / \Exp{\rhopar}}$ is at least an order of magnitude larger than $\sigma^2_{\rhoperp / \Exp{\rhoperp}}$, which is from the magnetic cushioning effect that suppresses fluctuations perpendicular to the mean-field. This effect is most strongly represented in the \texttt{M2MA01} simulation, where there is little contamination between the hydrodynamical and magnetised fluctuations due to large-scale shock mixing. 
     
    The key feature of these variances is that between $2\leq \M \leq 10$ the variance for both the components of the density field increases monotonically, as expected from the regular $\sigma^2_s - \M$ relation. This means that one, in theory, should be able to reduce a 2D column density map of an observed MC onto a 1D line and still measure the $\M$ using the variance of 1D field. We leave this interesting note for future studies. Thus, for future potential applications it is important to understand the projection effects on a stochastic field as it is integrated from 3D to 1D. 
    
    Projection effects play a significant role in this decomposition, since we perform two of them for each coordinate. Projections smooth fields, and act more strongly on small-scale features of the field, like highly-compressed, small-scale shocks that form in high-$\M$ turbulence \citep{Vazquez2001,Kim2005,Burkhart2012,Beattie2019a,Beattie2020}. For example, \citet{Beattie2019a} showed that the fractal dimension, $\D$, changed by 1 between the 3D and 2D projected density data for $\M \approx 2 - 4$, and 0.5 for $\M \approx 40 - 100$, where high-$\D$ corresponds to space-filling flow geometries. This means that projections smooth high-$\M$ more than they do low-$\M$ flows. 

    We quantify how the variances are influenced by our decomposition by plotting the ratio, $\sigma^2 / \sigma_{\rm 3D}^2$, where $\sigma_{\rm 3D}^2$ is the 3D variance, as a function of $\M$ in Figure~\ref{fig:1Dvariances}. Very little of the total 3D variance is preserved in our transformations. For the low-$\M$, it varies between $\approx 10^{-1}\sigma_{\rm 3D}^2$ and $< 10^{-3}\sigma_{\rm 3D}^2$ for $\rhopar$ and $\rhoperp$, respectively. As $\M$ increases the $\rhoperp$ variance ratio maps out the variance function from the top panel. This means that the smoothing acts more or less the same across the field, reducing the power in the fluctuations similarly for all $\M$. On the contrary, the $\rhopar$ variance ratio deviates significantly from the variance function, and is monotonically decreasing as $\M$ increases. 
    
    This analysis demonstrates the complexity of constructing models for the variances of projected data and now that we have established that the parallel and perpendicular density field holds different dynamical information through the PDFs, power spectra, and variances, we turn our attention to the 3D volume-weighted density statistics. This allows us to avoid the complications of the non-linear action of projections on the density fluctuations.  
